CODA-19: Using a Non-Expert Crowd to Annotate Research Aspects on 10,000+ Abstracts in the COVID-19 Open Research Dataset

This paper introduces CODA-19, a human-annotated dataset that codes the Background, Purpose, Method, Finding/Contribution, and Other sections of 10,966 English abstracts in the COVID-19 Open Research Dataset. CODA-19 was created by 248 crowd workers from Amazon Mechanical Turk within 10 days, and achieved labeling quality comparable to that of experts. Each abstract was annotated by nine different workers, and the final labels were acquired by majority vote. The inter-annotator agreement (Cohen's kappa) between the crowd and the biomedical expert (0.741) is comparable to inter-expert agreement (0.788). CODA-19's labels have an accuracy of 82.2% when compared to the biomedical expert's labels, while the accuracy between experts was 85.0%. Reliable human annotations help scientists access and integrate the rapidly accelerating coronavirus literature, and also serve as the battery of AI/NLP research, but obtaining expert annotations can be slow. We demonstrated that a non-expert crowd can be rapidly employed at scale to join the fight against COVID-19.

==> faq.tex <==
\section{Frequently Asked Questions (FAQs) from Workers}

\begin{enumerate}
    
\item \textbf{This text fragment has terms that I don't understand. What should I do?}\\
Please use the context in the article to figure out the focus. You can look up terms you don't know if you feel like you need to understand them.



\item \textbf{This text fragment is too short to mean anything. What should I do?}\\
If the text fragment is too short to have significant meanings, you could consider the entire sentence and answer based on the entire sentence.

\item \textbf{This text fragment is NOT in English. What should I do?}\\
If the whole fragment (or the majority of words in the fragment) is in Non-English, please label it as "Other". If the majority of the words in this fragment are in English with a few non-English words, please judge the label normally.

\item \textbf{I'm not sure if this should be a "background" or a "finding." How do I tell?}\\
When a sentence occurs in the earlier part of an article, and it is presented as a known fact or looks authoritative, it is often a "background" information.

\item \textbf{Q:} Do "potential applications of the proposed work" count as "background" or "purpose"?\\
\textbf{A:} It should be "background." The "purpose" refers to specific things the paper wants to achieve.

\item \textbf{If the article says it's a "literature review" (e.g., "We reviewed the literature" / "In this article, we review.." etc), would we classify those as finding/contribution or purpose?}\\
Most parts of a literature review paper should still be "background" or "purpose", and only the "insight" drew from a set of prior works can be viewed as a "finding/contribution".

\item \textbf{What should I do with the case study on a patient? Typically, it has a patient come in with a set of signs and symptoms in the ER, and then the patient gets assessed and diagnosed. The patient is admitted to the hospital ICU and tests are done and they may be diagnosed with something else.}\\
In such cases, please label the interventions done by the medical staff (e.g., CT scans, X-rays, and medications given) as "Method", and
the patient's final result (e.g. the patient's pneumonia resolved and he was released from the hospital) as "Finding/Contribution".

\end{enumerate}
